Leveraging The Topological Consistencies of Learning in Deep Neural Networks

Recently, methods have been developed to accurately predict the testing performance of a Deep Neural Network (DNN) on a particular task, given statistics of its underlying topological structure. However, further leveraging this newly found insight for practical applications is intractable due to the high computational cost in terms of time and memory. In this work, we define a new class of topological features that accurately characterize the progress of learning while being quick to compute during running time. Additionally, our proposed topological features are readily equipped for backpropagation, meaning that they can be incorporated in end-to-end training. Our newly developed practical topological characterization of DNNs allows for an additional set of applications. We first show we can predict the performance of a DNN without a testing set and without the need for high-performance computing. We also demonstrate our topological characterization of DNNs is effective in estimating task similarity. Lastly, we show we can induce learning in DNNs by actively constraining the DNN's topological structure. This opens up new avenues in constricting the underlying structure of DNNs in a meta-learning framework.

==> PAMI_Topology_work(5)/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> PAMI_Topology_work(5)/scratch.tex <==
# old table data performance

\begin{table*}[h] % Add the following just after the closing bracket on this line to specify a position for the table on the page: [h], [t], [b] or [p] - these mean: here, top, bottom and on a separate page, respectively
\centering % Centres the table on the page, comment out to left-justify
\scalebox{0.90}{
\begin{tabular}{l | c c c | c c c | c c c }
  &  \multicolumn{9}{c}{\textbf{Testing Performance Estimation}} 
\\  \cmidrule(l){1-10} \textbf{Synthetic}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc}} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{2D-Data}   &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}

\\ \textbf{Model}   &  Ours  &  Bench1  &  Ours+Bench1   &  Ours  &  Bench1  &  Ours+Bench1   &  Ours  &  Bench1  &  Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
synth fc6 & 73.32 $\pm$ 26.75  & -- --   & -- -- & 0.08 $\pm$ .02 & -- -- & -- -- & 0.05 $\pm$ 0.02   & -- -- & -- --
\\ synth fc8 & 80.53 $\pm$ 22.34 & -- -- & -- -- &  0.07 $\pm$ 0.02  & -- -- & -- -- & 0.05936 $\pm$ 0.02  & -- -- & -- --
\\   synth fc10 & 74.922 $\pm$ 26.41  & -- --  & -- -- & 0.35 $\pm$ 0.12 & -- -- & -- -- & 0.32 $\pm$ 0.13   & -- -- & -- --

\\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 2}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc }} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{Data}  &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 99.8 $\pm$ .7  &  -- -- & -- -- & 3.54 $\pm$ 1.30& -- -- & -- -- & 3.48 $\pm$ 1.35  & -- -- & -- --
 \\gconv3 & 99.9 $\pm$ 0.5   & -- -- & -- -- &  3.60 $\pm$ 1.74 & -- -- & -- -- & 3.60 $\pm$ 1.76  & -- -- & -- --
 \\ gconv4 & 99.81 $\pm$ 0.91 & -- --  & -- -- &  4.07 $\pm$ 1.50 & -- -- & -- -- & 3.77 $\pm$ 1.59  & -- -- & -- --
 
 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 4}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc }} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{Data}  &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 

\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 100.0 $\pm$ 0.0 & -- -- & -- -- & 4.53 $\pm$ 1.85 & -- -- & -- -- & 4.27 $\pm$ 2.21  & -- -- & -- --
 \\gconv3 & 99.91 $\pm$ 0.73 & -- -- & -- -- & 4.41 $\pm$ 1.74 & -- -- & -- -- & 4.35 $\pm$ 2.18  & -- -- & -- --
 \\ gconv4 & 100.0 $\pm$ 0.0   & -- -- & -- -- & 4.38 $\pm$ 1.75 & -- -- & -- -- & 4.13 $\pm$ 1.94  & -- -- & -- --
 


 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 8}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc }} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{Data}  &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 99.00 $\pm$ 1.0 & -- -- &  -- --& 4.40 $\pm$ 2.23 & -- -- & -- -- & 4.38 $\pm$ 2.53   & -- -- & -- --
 \\gconv3 & 99.00 $\pm$ 0.02 & -- -- & -- -- &  3.77 $\pm$ 1.67 & -- -- & -- -- & 3.99 $\pm$ 1.94 & -- -- & -- --
 \\ gconv4 & 100.0 $\pm$  0.0 & -- -- & -- -- & 4.50 $\pm$ 1.64 & -- -- & -- -- & 4.51 $\pm$ 1.74  & -- -- & -- --
 
 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Tiny 2}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc }} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{Data}  &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 tconv3 & 98.78 $\pm$ 2.25 & -- -- & -- --  &  6.77 $\pm$ 3.06 & -- -- & -- -- & 6.77 $\pm$ 3.06  & -- -- & -- --
\\tconv4 & 97.85 $\pm$ 3.02 & -- -- & -- -- & 7.17 $\pm$ 03.10 & -- -- & -- -- & 7.17 $\pm$ 3.10  & -- -- & -- --
\\tconv5 & 97.66 $\pm$ 3.04 & -- -- &   & 7.63 $\pm$ 3.506 & -- -- & -- -- & 7.63 $\pm$ 3.51  & -- -- & -- --
\\  \midrule
\end{tabular}}
\caption{Performance Estimation Results. The first 3 columns denote the average classification accuracy ( $\pm$ standard error) in predicting the intended model state for a given feature across samples and tasks. The next 6 columns present the mean absolute error in \% $\pm$ the standard error in estimating the testing accuracy and performance gap respectively across samples and tasks.} 

\label{tab:three}

\end{table*}


\begin{table*}[h] % Add the following just after the closing bracket on this line to specify a position for the table on the page: [h], [t], [b] or [p] - these mean: here, top, bottom and on a separate page, respectively
\centering % Centres the table on the page, comment out to left-justify
\scalebox{0.90}{
\begin{tabular}{l | c c c | c c c | c c c }
  &  \multicolumn{9}{c}{\textbf{Task Similarity}} 
\\  \cmidrule(l){1-10} \textbf{Synthetic}  &  \multicolumn{3}{c}{\textbf{Model Rank}} & \multicolumn{3}{c}{\textbf{Corr}} & \multicolumn{3}{c}{\textbf{Testing Improvement}}  
\\ \textbf{2D-Data}   &  \multicolumn{3}{c}{--} &  \multicolumn{3}{c}{--}  & \multicolumn{3}{c}{ (\%)} 

\\ \textbf{Model}   &  Ours  &  Bench1  &  Ours+Bench1   &  Ours  &  Bench1  &  Ours+Bench1   &  Ours  &  Bench1  &  Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
synth fc6 & --   --  & -- --   & -- -- & --  -- & -- -- & -- -- & -- --   & -- -- & -- --
\\ synth fc8 & --- & -- -- & -- -- &  ---  & -- -- & -- -- & -- --  & -- -- & -- --
\\   synth fc10 & -- --  & -- --  & -- -- & -- -- & -- -- & -- -- & -- --   & -- -- & -- --

\\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 2}  &  \multicolumn{3}{c}{\textbf{Model Rank}} &  \multicolumn{3}{c}{\textbf{Corr}}  &  \multicolumn{3}{c}{\textbf{Testing Improvement}}
\\ \textbf{2D-Data}   &  \multicolumn{3}{c}{--} & \multicolumn{3}{c}{--} & \multicolumn{3}{c}{(\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 7.82 $\pm$ 1.07   &  -- -- & -- -- & 0.276 $\pm$ 0.048  & -- -- & -- -- & 02.52 $\pm$ 00.6  & -- -- & -- --
 \\gconv3 & 7.49 $\pm$ 1.0432    & -- -- & -- -- &  0.391 $\pm$ 0.0523 & -- -- & -- -- & 02.83 $\pm$ 0.580 & -- -- & -- --
 \\ gconv4 & 8.78 $\pm$ 1.1  & -- --  & -- -- & 0.580 $\pm$ 0.039  & -- -- & -- -- & 03.57 $\pm$ 00.1  & -- -- & -- --
 
 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 4}  &   \multicolumn{3}{c}{\textbf{Model Rank}} & \multicolumn{3}{c}{\textbf{Corr}} & \multicolumn{3}{c}{\textbf{Testing Improvement}} 
\\ \textbf{Data}  &  \multicolumn{3}{c}{--} & \multicolumn{3}{c}{--} & \multicolumn{3}{c}{(\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 

\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 3.45 $\pm$ 0.894 & -- -- & -- -- & 0.548 $\pm$ 0.0810 & -- -- & -- -- & 0.035 $\pm$ 0.0127  & -- -- & -- --
 \\gconv3 & 3.81 $\pm$ 0.8702 & -- -- & -- -- & 0.556 $\pm$ 0.1253 & -- -- & -- -- & 0.02830 $\pm$ 0.0116  & -- -- & -- --
 \\ gconv4 & 4.36$\pm$ 0.883 & -- -- & -- -- & 0.5608 $\pm$ 04.9 & -- -- & -- -- & 01.8 $\pm$ 0.0174  & -- -- & -- --
 


 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 8}  &   \multicolumn{3}{c}{\textbf{Model Rank}} & \multicolumn{3}{c}{\textbf{Corr}} & \multicolumn{3}{c}{\textbf{Testing Improvement}}  
\\ \textbf{Data}  &  \multicolumn{3}{c}{--} & \multicolumn{3}{c}{--} & \multicolumn{3}{c}{(\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 &  1.4 $\pm$ 0.21908  & -- -- &  -- --& 0.981 $\pm$ 0.0052 & -- -- & -- -- & 04.42$\pm$ 0.78   & -- -- & -- --
 \\gconv3 & 1.0 $\pm$ 0 & -- -- & -- -- &  0.9957 $\pm$ 0.00138 & -- -- & -- -- &  06.1 $\pm$ 00.489  & -- -- & -- --
 \\ gconv4 & 1.5 $\pm$ 0.431 & -- -- & -- -- & .976 $\pm$ .0032 & -- -- & -- -- & 05.23 $\pm$ 1.44  & -- -- & -- --
 
 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Tiny 2}  &   \multicolumn{3}{c}{\textbf{Model Rank}} &  \multicolumn{3}{c}{\textbf{Corr}} & \multicolumn{3}{c}{\textbf{Testing Improvement}} 
\\ \textbf{Data}  &  \multicolumn{3}{c}{(--)} & \multicolumn{3}{c}{--} & \multicolumn{3}{c}{(\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 tconv3 &-- -- & -- -- & -- --  &  -- -- & -- -- & -- -- & -- --  & -- -- & -- --
\\tconv4 & -- -- & -- -- & -- -- & -- -- & -- -- & -- -- & -- --  & -- -- & -- --
\\tconv5 & -- -- & -- -- &  -- --  & -- -- & -- -- & -- -- & -- --  & -- -- & -- --
\\  \midrule
\end{tabular}}
\caption{To evaluate our model $h'''$  we determine the rank our current model selection in comparison to the others in terms of fine-tuning performance.  We also examine how our linear models correlate with the actual predicted testing performance. Lastly, we examine how our models compare to a randomly selected model in the bank of pre-trained models and record the average testing improvement compared to the randomly selected baseline. $n_{models}$ denotes the number of folds in the cross validation procedure. This implies we could choose from $n_{models}-1$ models after each linear model $h'''$ is constructed. Standard error is recorded to the right of each statistic.} 

\label{tab:template}

\end{table*}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> scratch.tex <==
# old table data performance

\begin{table*}[h] % Add the following just after the closing bracket on this line to specify a position for the table on the page: [h], [t], [b] or [p] - these mean: here, top, bottom and on a separate page, respectively
\centering % Centres the table on the page, comment out to left-justify
\scalebox{0.90}{
\begin{tabular}{l | c c c | c c c | c c c }
  &  \multicolumn{9}{c}{\textbf{Testing Performance Estimation}} 
\\  \cmidrule(l){1-10} \textbf{Synthetic}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc}} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{2D-Data}   &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}

\\ \textbf{Model}   &  Ours  &  Bench1  &  Ours+Bench1   &  Ours  &  Bench1  &  Ours+Bench1   &  Ours  &  Bench1  &  Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
synth fc6 & 73.32 $\pm$ 26.75  & -- --   & -- -- & 0.08 $\pm$ .02 & -- -- & -- -- & 0.05 $\pm$ 0.02   & -- -- & -- --
\\ synth fc8 & 80.53 $\pm$ 22.34 & -- -- & -- -- &  0.07 $\pm$ 0.02  & -- -- & -- -- & 0.05936 $\pm$ 0.02  & -- -- & -- --
\\   synth fc10 & 74.922 $\pm$ 26.41  & -- --  & -- -- & 0.35 $\pm$ 0.12 & -- -- & -- -- & 0.32 $\pm$ 0.13   & -- -- & -- --

\\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 2}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc }} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{Data}  &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 99.8 $\pm$ .7  &  -- -- & -- -- & 3.54 $\pm$ 1.30& -- -- & -- -- & 3.48 $\pm$ 1.35  & -- -- & -- --
 \\gconv3 & 99.9 $\pm$ 0.5   & -- -- & -- -- &  3.60 $\pm$ 1.74 & -- -- & -- -- & 3.60 $\pm$ 1.76  & -- -- & -- --
 \\ gconv4 & 99.81 $\pm$ 0.91 & -- --  & -- -- &  4.07 $\pm$ 1.50 & -- -- & -- -- & 3.77 $\pm$ 1.59  & -- -- & -- --
 
 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 4}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc }} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{Data}  &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 

\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 100.0 $\pm$ 0.0 & -- -- & -- -- & 4.53 $\pm$ 1.85 & -- -- & -- -- & 4.27 $\pm$ 2.21  & -- -- & -- --
 \\gconv3 & 99.91 $\pm$ 0.73 & -- -- & -- -- & 4.41 $\pm$ 1.74 & -- -- & -- -- & 4.35 $\pm$ 2.18  & -- -- & -- --
 \\ gconv4 & 100.0 $\pm$ 0.0   & -- -- & -- -- & 4.38 $\pm$ 1.75 & -- -- & -- -- & 4.13 $\pm$ 1.94  & -- -- & -- --
 


 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 8}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc }} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{Data}  &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 99.00 $\pm$ 1.0 & -- -- &  -- --& 4.40 $\pm$ 2.23 & -- -- & -- -- & 4.38 $\pm$ 2.53   & -- -- & -- --
 \\gconv3 & 99.00 $\pm$ 0.02 & -- -- & -- -- &  3.77 $\pm$ 1.67 & -- -- & -- -- & 3.99 $\pm$ 1.94 & -- -- & -- --
 \\ gconv4 & 100.0 $\pm$  0.0 & -- -- & -- -- & 4.50 $\pm$ 1.64 & -- -- & -- -- & 4.51 $\pm$ 1.74  & -- -- & -- --
 
 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Tiny 2}  &  \multicolumn{3}{c}{\textbf{Model State}} & \multicolumn{3}{c}{\textbf{Testing Acc }} & \multicolumn{3}{c}{\textbf{Performance Gap}}
\\ \textbf{Data}  &  \multicolumn{3}{c}{Mean Acc (\%)} & \multicolumn{3}{c}{ MAE (\%)} & \multicolumn{3}{c}{MAE (\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 tconv3 & 98.78 $\pm$ 2.25 & -- -- & -- --  &  6.77 $\pm$ 3.06 & -- -- & -- -- & 6.77 $\pm$ 3.06  & -- -- & -- --
\\tconv4 & 97.85 $\pm$ 3.02 & -- -- & -- -- & 7.17 $\pm$ 03.10 & -- -- & -- -- & 7.17 $\pm$ 3.10  & -- -- & -- --
\\tconv5 & 97.66 $\pm$ 3.04 & -- -- &   & 7.63 $\pm$ 3.506 & -- -- & -- -- & 7.63 $\pm$ 3.51  & -- -- & -- --
\\  \midrule
\end{tabular}}
\caption{Performance Estimation Results. The first 3 columns denote the average classification accuracy ( $\pm$ standard error) in predicting the intended model state for a given feature across samples and tasks. The next 6 columns present the mean absolute error in \% $\pm$ the standard error in estimating the testing accuracy and performance gap respectively across samples and tasks.} 

\label{tab:three}

\end{table*}


\begin{table*}[h] % Add the following just after the closing bracket on this line to specify a position for the table on the page: [h], [t], [b] or [p] - these mean: here, top, bottom and on a separate page, respectively
\centering % Centres the table on the page, comment out to left-justify
\scalebox{0.90}{
\begin{tabular}{l | c c c | c c c | c c c }
  &  \multicolumn{9}{c}{\textbf{Task Similarity}} 
\\  \cmidrule(l){1-10} \textbf{Synthetic}  &  \multicolumn{3}{c}{\textbf{Model Rank}} & \multicolumn{3}{c}{\textbf{Corr}} & \multicolumn{3}{c}{\textbf{Testing Improvement}}  
\\ \textbf{2D-Data}   &  \multicolumn{3}{c}{--} &  \multicolumn{3}{c}{--}  & \multicolumn{3}{c}{ (\%)} 

\\ \textbf{Model}   &  Ours  &  Bench1  &  Ours+Bench1   &  Ours  &  Bench1  &  Ours+Bench1   &  Ours  &  Bench1  &  Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
synth fc6 & --   --  & -- --   & -- -- & --  -- & -- -- & -- -- & -- --   & -- -- & -- --
\\ synth fc8 & --- & -- -- & -- -- &  ---  & -- -- & -- -- & -- --  & -- -- & -- --
\\   synth fc10 & -- --  & -- --  & -- -- & -- -- & -- -- & -- -- & -- --   & -- -- & -- --

\\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 2}  &  \multicolumn{3}{c}{\textbf{Model Rank}} &  \multicolumn{3}{c}{\textbf{Corr}}  &  \multicolumn{3}{c}{\textbf{Testing Improvement}}
\\ \textbf{2D-Data}   &  \multicolumn{3}{c}{--} & \multicolumn{3}{c}{--} & \multicolumn{3}{c}{(\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 7.82 $\pm$ 1.07   &  -- -- & -- -- & 0.276 $\pm$ 0.048  & -- -- & -- -- & 02.52 $\pm$ 00.6  & -- -- & -- --
 \\gconv3 & 7.49 $\pm$ 1.0432    & -- -- & -- -- &  0.391 $\pm$ 0.0523 & -- -- & -- -- & 02.83 $\pm$ 0.580 & -- -- & -- --
 \\ gconv4 & 8.78 $\pm$ 1.1  & -- --  & -- -- & 0.580 $\pm$ 0.039  & -- -- & -- -- & 03.57 $\pm$ 00.1  & -- -- & -- --
 
 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 4}  &   \multicolumn{3}{c}{\textbf{Model Rank}} & \multicolumn{3}{c}{\textbf{Corr}} & \multicolumn{3}{c}{\textbf{Testing Improvement}} 
\\ \textbf{Data}  &  \multicolumn{3}{c}{--} & \multicolumn{3}{c}{--} & \multicolumn{3}{c}{(\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 

\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 & 3.45 $\pm$ 0.894 & -- -- & -- -- & 0.548 $\pm$ 0.0810 & -- -- & -- -- & 0.035 $\pm$ 0.0127  & -- -- & -- --
 \\gconv3 & 3.81 $\pm$ 0.8702 & -- -- & -- -- & 0.556 $\pm$ 0.1253 & -- -- & -- -- & 0.02830 $\pm$ 0.0116  & -- -- & -- --
 \\ gconv4 & 4.36$\pm$ 0.883 & -- -- & -- -- & 0.5608 $\pm$ 04.9 & -- -- & -- -- & 01.8 $\pm$ 0.0174  & -- -- & -- --
 


 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Grey 8}  &   \multicolumn{3}{c}{\textbf{Model Rank}} & \multicolumn{3}{c}{\textbf{Corr}} & \multicolumn{3}{c}{\textbf{Testing Improvement}}  
\\ \textbf{Data}  &  \multicolumn{3}{c}{--} & \multicolumn{3}{c}{--} & \multicolumn{3}{c}{(\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 gconv2 &  1.4 $\pm$ 0.21908  & -- -- &  -- --& 0.981 $\pm$ 0.0052 & -- -- & -- -- & 04.42$\pm$ 0.78   & -- -- & -- --
 \\gconv3 & 1.0 $\pm$ 0 & -- -- & -- -- &  0.9957 $\pm$ 0.00138 & -- -- & -- -- &  06.1 $\pm$ 00.489  & -- -- & -- --
 \\ gconv4 & 1.5 $\pm$ 0.431 & -- -- & -- -- & .976 $\pm$ .0032 & -- -- & -- -- & 05.23 $\pm$ 1.44  & -- -- & -- --
 
 \\  \cmidrule(l){1-1} \cmidrule(l){2-10} \textbf{Tiny 2}  &   \multicolumn{3}{c}{\textbf{Model Rank}} &  \multicolumn{3}{c}{\textbf{Corr}} & \multicolumn{3}{c}{\textbf{Testing Improvement}} 
\\ \textbf{Data}  &  \multicolumn{3}{c}{(--)} & \multicolumn{3}{c}{--} & \multicolumn{3}{c}{(\%)}
\\ \textbf{Model}  &  Ours    &  Bench 1 &   Ours + Bench1 & Ours & Bench1 & Ours+Bench1 & Ours & Bench1 & Ours+Bench1 
\\ \cmidrule(l){1-1} \cmidrule(l){2-10} 
 tconv3 &-- -- & -- -- & -- --  &  -- -- & -- -- & -- -- & -- --  & -- -- & -- --
\\tconv4 & -- -- & -- -- & -- -- & -- -- & -- -- & -- -- & -- --  & -- -- & -- --
\\tconv5 & -- -- & -- -- &  -- --  & -- -- & -- -- & -- -- & -- --  & -- -- & -- --
\\  \midrule
\end{tabular}}
\caption{To evaluate our model $h'''$  we determine the rank our current model selection in comparison to the others in terms of fine-tuning performance.  We also examine how our linear models correlate with the actual predicted testing performance. Lastly, we examine how our models compare to a randomly selected model in the bank of pre-trained models and record the average testing improvement compared to the randomly selected baseline. $n_{models}$ denotes the number of folds in the cross validation procedure. This implies we could choose from $n_{models}-1$ models after each linear model $h'''$ is constructed. Standard error is recorded to the right of each statistic.} 

\label{tab:template}

\end{table*}
